Overdetermined 2D Systems Invariant in One Direction and Their Transfer Functions

In this work we develop a theory of Vessels. This object arises in the study of overdetermined 2D systems invariant in one of the variables, which are usually called time invariant. To each overdetermined time invariant 2D systems there is associated a vessel, which is a collection of system operators satisfying certain relations and vise versa. Such an invariance forces the theory of vessels to resemble a constant (classical) 1D case and as a result many notions are naturally redefined and most theorems are reproved in this setting. The notion of transfer function and its connection to the overdetermined 2D time invariant system (and the corresponding vessel) is one of the topics of this work. It is well known that multiplicative structure of a transfer function of a 1D system is closely connected to the decomposition of the state space into invariant subspaces of the state operator and we generalize this result to a wider class of functions. This class (denoted by $\boldsymbol {\mathcal I}$) arises as a class of transfer functions, which intertwine solutions of ODEs with spectral parameters. At the end we present solution of factorization problems for finite dimensional case.

==> Conclusions.tex <==
% -------------------------------- Adjoint system ----------------------------------------------
\subsection{Adjoint system}
The notion of adjoint system is very useful in system theory. It is obtained from a simple observation
that applying adjoint to the vessel conditions gives rise to a new set of conditions on
adjoint operators, which is almost vessel conditions. Moreover $(\Sigma^*)^*$ is actually
$\Sigma$ by a trivial change of coordinates $x \rightarrow -x$ on the state space. Here is the precise definition.
Given a system in the differential form
\begin{equation} \label{eq:DSigma}
    D\Sigma: \left\{ \begin{array}{lll}
    \frac{\partial}{\partial t_1}x(t_1,t_2) = A_1(t_2) x(t_1,t_2) + \widetilde{B}(t_2) ~\sigma_1(t_2) ~u(t_1,t_2) \\
    \frac{\partial}{\partial t_2}x(t_1,t_2) = A_2(t_2) x(t_1,t_2) + \widetilde{B}(t_2) ~\sigma_2(t_2) ~u(t_1,t_2) \\
    y(t_1,t_2) = D(t_2) u(t_1,t_2) + C(t_2) x(t_1,t_2)
    \end{array} \right.
\end{equation}
and associated vessel
\[ \mathfrak{V} = (A_1(t_2), A_2(t_2),\widetilde{B}(t_2),C(t_2), D(t_2),\widetilde D(t_2);
        \sigma_1(t_2), \sigma_2(t_2), \gamma(t_2), \sigma_{1*}(t_2), \sigma_{2*}(t_2)\gamma_*(t_2);
        \mathcal H, \mathcal{E},\mathcal E_*, \mathcal{\widetilde E},\mathcal{\widetilde E_*})
\]
it is natural to introduce the \textit{adjoint system}:
\begin{equation} \label{eq:systemAdj}
    D\Sigma^*: \left\{ \begin{array}{lll}
    -\frac{\partial}{\partial t_1}x_*(t_1,t_2) = A_1^*(t_2) ~x_*(t_1,t_2) + C^*(t_2) \sigma^*_{1*} u_*(t_1,t_2) \\[5pt]
    -\frac{\partial}{\partial t_2}x_*(t_1,t_2) = A_2^*(t_2) ~x_*(t_1,t_2) + C^*(t_2) \sigma^*_{2*} u_*(t_1,t_2) \\[5pt]
    y_*(t_1,t_2) = \widetilde B^*~ x_*(t_1,t_2)  + \widetilde D^*(t_2)~ u_*(t_1,t_2)[[,]]
    \end{array} \right.
\end{equation}
which is associated to the vessel $\mathfrak{V^*}$ given by
\[ \mathfrak{V^*} =
(-A_1^*, -A_2^*, -C^*, \widetilde B^*, \widetilde D^*, D^*;
\sigma^*_{1*}, \sigma^*_{2*}, -\gamma_*^* - \frac{d}{dt_2}
\sigma_{1*}^*, \sigma^*_1, \sigma^*_2, -\gamma^* - \frac{d}{dt_2}
\sigma_1^*; \mathcal{H}, \widetilde{\mathcal E}_*,
\widetilde{\mathcal E}_*, \mathcal{E}_*, \mathcal{E}),
\]
where all the operators are functions of $t_2$ and satisfy the following axioms:
\[ \begin{array}{lllllll}
    \frac{d}{dt_2} A_1^* = A_1^* A_2^* - A_2^* A_1^* \\
   -\frac{d}{dt_2} \big(C^* \sigma^*_{1*} \big) - A_2^* C^* \sigma^*_{1*} + A_1^* C^* \sigma^*_{2*}
   + C^* (\gamma_*^*+\frac{d}{dt_2} \sigma_{1*}^*) = 0 \\
    \frac{d}{dt_2} \big(\sigma_1^* \widetilde B^* \big) - \sigma_1^* \widetilde B^* A_2^* +
    \sigma_2^* \widetilde B A_1^* + \gamma^* \widetilde B^* = 0 \\
   \sigma^*_1 \widetilde D^* = D^* \sigma^*_{1*}, ~~ \sigma^*_2 \widetilde D^* = D^* \sigma^*_{2*} \\
   D^* (-\gamma^*_* -\frac{d}{dt_2} \sigma_{1*}^*) = -\sigma^*_2 \widetilde B^* C^* \sigma^*_{1*} +
   \sigma^*_1 \widetilde B^* C^* \sigma^*_{2*} - \sigma^*_1 \frac{d}{dt_2} \widetilde D^* - (\gamma^* +\frac{d}{dt_2} \sigma_1^*)\widetilde D^*.
   \end{array}
\]
Moreover, the transfer function of the adjoint vessel $S_*(\mu,t_2)$ maps solutions of the \textit{adjoint input} ODE
\begin{equation} \label{eq:InCC*} [\sigma^*_{2*} \mu - \sigma^*_{1*} \dfrac{d}{dt_2} -
\gamma^*_* - \frac{d}{dt_2} \sigma_{1*}^*] u_*(t_2) = 0
\end{equation}
with the spectral parameter $\mu$ to solutions of the \textit{adjoint output} ODE
\begin{equation} \label{eq:OutCC*} [\sigma^*_2 \mu - \sigma^*_1 \dfrac{d}{dt_2} -
\gamma^*-\frac{d}{dt_2} \sigma_1^*] y_*(t_2) = 0
\end{equation}
with the same spectral parameter. In the language of fundamental
matrices, if one denotes the fundamental solution for $u_*(t_2),
y_*(t_2)$ as $\Psi(\mu,t_2, t_2^0)$ and $\Psi_*(\mu,t_2, t_2^0)$[[,]]
respectively, then (similarly to (\ref{eq:SInttw}))
\[ S_*(\mu, t_2) \Psi(\mu,t_2,\tau_2) =
\Psi_*(\mu,t_2,\tau_2) S_*(\mu, \tau_2)
\]
Notice also that the equation for $S_*(\lambda, t_2)$ similar to
(\ref{eq:S}) is:
\[ S_*(\mu, t_2) = \widetilde D^* - \widetilde B^* (\mu I +
A_1^*)^{-1} C^* \sigma^*_{1*}
\]
And as in the case of constant operators[[,]] one obtains that
$\mathfrak{V^*}$ is a vessel iff $\mathfrak{V}$ is. And as we mentioned before[[,]]
$\mathfrak{V^*}^*$ is the same as $\mathfrak V$ after a trivial
change of coordinates $x \rightarrow -x$ on the state space.

\noindent \textbf{Remarks:}
\begin{enumerate}
\item It is also simple to check that $\sigma_{1*}^* \Phi_*^{-1*}(\lambda, t_2, t_2^0)$ and
$\Psi(-\bar\lambda, t_2, t_2^0)$ satisfy the same differential equation. Since they are fundamental
matrices it is possible iff
\begin{eqnarray}\label{eq:Phi*Psi}
 \sigma_{1*}^{-1*} \Phi_*^{-1*}(\lambda, t_2, t_2^0) = \Psi(-\bar\lambda, t_2, t_2^0)  \sigma_{1*}^{-1*} \\
 \label{eq:PhiPsi*} \sigma_1^{-1*} \Phi^{-1*}(\lambda, t_2, t_2^0) = \Psi_*(-\bar\lambda, t_2, t_2^0)  \sigma_1^{-1*}
\end{eqnarray}
\item This connection between $\Phi$ and $\Psi$ fundamental matrices means that the following connection
between transfer functions [[has]] to be satisfied:
\begin{equation} \label{eq:SS*}
 S(\lambda, t_2) =  \sigma_{1*}^{-1} S^*_*(-\bar\lambda, t_2) \sigma_1
\end{equation}
One can easily verify the last formula, using the vessel conditions and the formulas for
$S(\lambda, t_2)$, $S^*_*(-\bar\lambda, t_2)$:
\[ \begin{array}{lllllll}
  \sigma_{1*}^{-1} S^*_*(-\bar\lambda, t_2) \sigma_1 =
  \sigma_{1*}^{-1} \big[ \widetilde D^* - \widetilde B^* (-\bar\lambda I +
A_1^*)^{-1} C^* \sigma^*_{1*} \big]^* \sigma_1 = \\
 ~~~~ = \sigma_{1*}^{-1} [\widetilde D - \sigma_{1*} C(-\lambda I + A_1)^{-1} \widetilde B]\sigma_1 =
    \sigma_{1*}^{-1} \widetilde D \sigma_1 - C(-\lambda I + A_1)^{-1} \widetilde B \sigma_1 = \\
 ~~~~ = D + C (\lambda I - A_1)^{-1} \widetilde B \sigma_1 = S(\lambda, t_2).
\end{array} \]
\item For values of $\lambda$ out of the spectrum of $A_1(t_2)$ (which is independent of $t_2$),
we claim that $S(\lambda, t_2)$ is invertible iff $S^*_*(-\bar\lambda, t_2)$ is and from (\ref{eq:SS*})
we conclude that
\[ S(\lambda, t_2)^{-1} = \sigma_1^{-1} S^{-1*}_*(-\bar\lambda, t_2) \sigma_{1*} \]
\end{enumerate}

